Inferring potential landscapes from noisy trajectories

While particle trajectories encode information on their governing potentials, potentials can be challenging to robustly extract from trajectories. Measurement errors may corrupt a particle's position, and sparse sampling of the potential limits data in higher-energy regions such as barriers. We develop a Bayesian method to infer potentials of arbitrary shape alongside measurement noise. As an alternative to Gaussian process priors over potentials, we introduce structured kernel interpolation to the Natural Sciences which allows us to extend our analysis to large data sets. Our method is validated on 1D and 2D experimental trajectories for particles in a feedback trap.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> old/experiments.tex <==
\section{Experiments}

A few data sets would help demonstrate that the method works:
\begin{itemize}
    \item \textbf{Data with no added measurement noise.} This serves as a proof of principle. Bechhoeffer lab has already provided sample data sets to train on. We accurately learned the force using these data sets. Verification of the algorithm was achieved by comparing the force learned using the Boltzmann histogram method. For a full manuscript it would be good to have the following data sets:\\
    \begin{itemize}
        \item Trajectory from a simple harmonic well\\
        \item Trajectory from an asymmetric double well (already provided)\\
        \item (Optional) Trajectory from a tilted washboard potential. This would be interesting because it would allow us to use our method in a non-equilibrium system, where the Boltzmann histogram method fundamentally will fail.
    \end{itemize}
    
    For each of these data sets, the depths of the well, mass, friction coefficient, etc., should be similar to the values used in the data sets that Bechhoeffer lab has already provided. Let that data set serve as a good example.
    
    \item \textbf{Data with measurement noise.} This would be analyzable using the algorithm proposed in this write up. For a full manuscript we would want to analyze the same potentials listed above, but with measurement noise at variable levels. We can quantify the size of the measurement noise (Eq.~\ref{likelihood}) in relation to either the width of the potential wells, or the size of the thermal kicks (Eq.~\ref{langevin}). We would want to analyze each of the data sets above, but with measurement noise added in quantities ranging from low to high. For example, something like the following is what we have in mind:\\
    \begin{itemize}
        \item $\sigma =$ one tenth the width of a well\\
        \item $\sigma =$ half the width of a well\\
        \item $\sigma =$ the width of a well\\
        \item $\sigma =$ twice the width of a well\\
    \end{itemize}
    or if ``width of a well'' is too abstract, something like this would also suffice:
    \begin{itemize}
        \item $\sigma = .1\left(\frac{2\tau kT}{\zeta}\right)$\\
        \item $\sigma = .5\left(\frac{2\tau kT}{\zeta}\right)$\\
        \item $\sigma = \left(\frac{2\tau kT}{\zeta}\right)$\\
        \item $\sigma = 2\left(\frac{2\tau kT}{\zeta}\right)$
    \end{itemize}
    Note that this serves as a guideline for what we have in mind, but not necessarily as a template for exact values of $\sigma$.
    
    \item \textbf{(Optional)} We have additional ideas we can add to the model presented in this write up. These include generalizing the model to 2D, generalizing the model to 3D, and generalizing the model to allow time dependent potentials. If possible these additional data sets could be useful:
    \begin{itemize}
        \item \textbf{(Optional)} Trajectory from a 2D or 3D simple harmonic well\\
        \item \textbf{(Optional)} Trajectory from a 2D or 3D double well\\
        \item \textbf{(Optional)} Trajectory from a 1D time varying potential
    \end{itemize}
    
    Note that we have not yet formalized the method to analyze these additional optional data sets (mostly because we do not know if it is possible to collect the data needed to test them), however, in principle, the only major change that would go into the model would be a slight modification to equation~\ref{hyperstuff}.
\end{itemize}
